TextMesh: Generation of Realistic 3D Meshes From Text Prompts

The ability to generate highly realistic 2D images from mere text prompts has recently made huge progress in terms of speed and quality, thanks to the advent of image diffusion models. Naturally, the question arises if this can be also achieved in the generation of 3D content from such text prompts. To this end, a new line of methods recently emerged trying to harness diffusion models, trained on 2D images, for supervision of 3D model generation using view dependent prompts. While achieving impressive results, these methods, however, have two major drawbacks. First, rather than commonly used 3D meshes, they instead generate neural radiance fields (NeRFs), making them impractical for most real applications. Second, these approaches tend to produce over-saturated models, giving the output a cartoonish looking effect. Therefore, in this work we propose a novel method for generation of highly realistic-looking 3D meshes. To this end, we extend NeRF to employ an SDF backbone, leading to improved 3D mesh extraction. In addition, we propose a novel way to finetune the mesh texture, removing the effect of high saturation and improving the details of the output 3D mesh.

==> sections/preliminiaries.tex <==
\section{Preliminaries}

This section serves to introduce all the relevant knowledge around Neural Radiance Fields, required to understand our propose method.

\subsection{Neural Radiance Fields}
At the core, a neural radiance field is a continuous mapping from a 3D location $\mathbf{x} \in \mathbb{R}^3$ and a ray viewing direction
 $\mathbf{d} \in \mathbb{S}^2$ 
to an RGB color $\mathbf{c} \in \left[ 0, 1 \right]^3$ and volume density $\sigma \in \reals^+$. It can be formulated as,
\begin{equation}
\left[\mathbf{c}, \sigma\right] = F_{\theta} \left(\gamma_{\textit{x}}(\mathbf{x}), \gamma_{\textit{d}}({\mathbf{d}})\right) \,
\label{eq:mlp}
\end{equation}
where $F$ is modeled as an MLP with learnable parameters  $\theta$, and $\gamma: \reals^{3} \rightarrow \reals^{N}$ is a positional encoding of the input $\mathbf{x}$ required to capture high frequencies.


Given a camera pose $P_i = [R_i, t_i] \in SE(3)$, each pixel coordinate $\mathbf{p} \in \reals^{2}$  determines a ray in the world coordinate system, whose origin is the camera center of projection $\mathbf{o}_{i} = \mathbf{t}_i$ and direction is defined as $\mathbf{d}_{i, \text{p}} = R_i K_i^{-1}\bar{\mathbf{p}}$. We can express a 3D point along the viewing ray associated with $\mathbf{p}$ at depth $t$ as $\mathbf{r}_{i, \text{p}} (t) = \mathbf{o}_i + t \mathbf{d}_{i, \text{p}}$. 
To render the color $\hat{\mathbf{I}}_{i, \text{p}} \in \left[0, 1\right]^3$ at pixel $\mathbf{p}$, we sample $M$ discrete depth values $t_m$ along the ray within the near and far plane $\left[t_n, t_f \right]$, and query $F_{\theta}$ at the associated 3D points. The corresponding predicted color and volume density values $\left\{(\mathbf{c}_m, \sigma_m  ) \right\}_{m=1}^M$ are then composited as,
\begin{align}
\hat{\mathbf{I}}_{i, \text{p}} &= \hat{I}(\mathbf{p}; \theta, P_i) = \sum_{m=1}^{M} \alpha_m\mathbf{c}_m \,, \label{eq:volume_rendering} \\
\text{where} \quad \alpha_m &= T_m\left(1 - \exp(-\sigma_m\delta_m)\right) \,, \label{eq:rendering_weight} \\
T_m &= \exp \left( -\sum_{m'=1}^{m} \sigma_{m'}\delta_{m'}\right)\,. \label{eq:transmittance}
\end{align}

where $T_m$ denotes the accumulated transmittance along the ray from $t_n$ to $t_m$, and $\delta_m = t_{m+1} - t_m$ is the distance between adjacent samples. 






